Verification of Sequential Convex Programming for Parametric Non-convex Optimization

We introduce a verification framework to exactly verify the worst-case performance of sequential convex programming (SCP) algorithms for parametric non-convex optimization. The verification problem is formulated as an optimization problem that maximizes a performance metric (e.g., the suboptimality after a given number of iterations) over parameters constrained to be in a parameter set and iterate sequences consistent with the SCP update rules. Our framework is general, extending the notion of SCP to include both conventional variants such as trust-region, convex-concave, and prox-linear methods, and algorithms that combine convex subproblems with rounding steps, as in relaxing and rounding schemes. Unlike existing analyses that may only provide local guarantees under limited conditions, our framework delivers global worst-case guarantees--quantifying how well an SCP algorithm performs across all problem instances in the specified family. Applications in control, signal processing, and operations research demonstrate that our framework provides, for the first time, global worst-case guarantees for SCP algorithms in the parametric setting.

==> cover/siopt_coverletter.tex <==
% !TeX root = siopt_coverletter.tex
% !TEX program = pdflatex
\input{siopt_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

SIAM Journal on Optimization

\bigskip

Dear Editors:

We are writing to submit our manuscript ``\red{Verification of Sequential Convex Programming for Parametric Non-convex Optimization}'' to \emph{SIAM Journal on Optimization}.

Our manuscript introduces a \red{verification framework to exactly verify the worst-case performance of sequential convex programming algorithms for parametric non-convex optimization}.
The verification problem is formulated as an optimization problem that maximizes a performance metric ({\it e.g.}, the suboptimality after a given number of iterations) over parameters constrained to be in a parameter set and iterate sequences consistent with the sequential convex programming update rules. 
This is important because sequential convex programming methods are widely used in practice to solve challenging non-convex optimization problems but typically lack global worst-case performance guarantees.
We showcase our framework on applications in control, signal processing, and operations research, demonstrating that it provides, for the first time, global worst-case guarantees for sequential convex programming algorithms in the parametric setting.
% This is important because many applications require solving parametric convex optimization problems in real-time.
% Additionally, in safety-critical domains, it is essential to certify the worst-case performance within a budget of iterations.
% We obtain a strong form of robustness guarantee---certification of worst-case performance over all parameters within a set after a given number of iterations---through regularization-based training.
% The regularization term is derived from the performance estimation problem framework based on semidefinite programming, in which the hyperparameters appear as problem data.
% We use gradient-based training to learn the hyperparameters for a variety of first-order methods.
% We apply our learning framework to numerous examples in control, statistics, and signal processing, and show that our method dramatically improves the quality of the solution within a given budget of iterations.
% Our approach is highly data-efficient since we only use ten training instances in each of our examples.



We suggest the following associate editors and referees for our submission.

Associate Editors:
% \begin{itemize}
%     \item \red{Silvia Villa}, University of Genova (villa@dima.unige.it)
%     \item \red{Quentin Berthet}, Google DeepMind (qberthet@google.com)
%     \item \red{Stefanie Jegelka}, Massachusetts Institute of Technology (stefje@csail.mit.edu)
%     \item \red{Jean-Philippe Vert}, Owkin (jean-philippe.vert@m4x.org)
%     \item \red{Shiqian Ma}, Rice University (sqma@rice.edu)
% \end{itemize}
\begin{itemize}
    \item \red{Frank E. Curtis}, Lehigh University (frank.e.curtis@lehigh.edu)
    \item \red{Stephen J. Wright}, University of Wisconsin-Madison (swright@cs.wisc.edu)
    \item \red{Andreas Wächter}, Northwestern University (andreas.waechter@northwestern.edu)
    \item \red{Coralia Cartis}, University of Oxford (Coralia.Cartis@maths.ox.ac.uk)
    % \item \red{Shiqian Ma}, Rice University (sqma@rice.edu)
\end{itemize}

Reviewers:
% \begin{itemize}
%     \item \red{Joe Marino}, Google DeepMind (josephmarino@google.com)
%     \item \red{Atlas Wang}, University of Texas, Austin (atlaswang@utexas.edu)
%     \item \red{Ernest Ryu}, Seoul National University (ernestryu@snu.ac.kr)
%     \item \red{Yisong Yue}, California Institute of Technology (yyue@caltech.edu)
%     \item \red{Pontus Giselsson}, Lund University (pontusg@control.lth.se)
% \end{itemize}
\begin{itemize}
    \item \red{Steven Diamond}, Gridmatic (steven@gridmatic.com)
    \item \red{Abhishek Cauligi}, Johns Hopkins University (cauligi@jh.edu)
    \item \red{Paul Grigas}, University of California-Berkeley (pgrigas@berkeley.edu)
    \item \red{Madeleine Udell}, Stanford University (udell@stanford.edu)
    % \item \red{Brendan O'Donoghue}, Google DeepMind (bodonoghue85@gmail.com)
    \item \red{Ján Drgoňa}, Johns Hopkins University (jdrgona1@jh.edu)
    % \item \red{Atlas Wang}, University of Texas, Austin (atlaswang@utexas.edu)
\end{itemize}

Our submission has the following keywords: \red{parametric optimization}, \red{non-convex optimization}, \red{sequential convex programming}, \red{computer-assisted optimization analysis}.

As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. 
Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{SIAM Journal on Optimization}.

\bigskip

Sincerely,

\medskip

Rajiv Sambharya (University of Pennsylvania)\\
Nikolai Matni (University of Pennsylvania)\\
George Pappas (University of Pennsylvania)

\end{document}
